Discrete and higher-form symmetries in SCFTs from wrapped M5-branes

We analyze topological mass terms of BF type arising in supersymmetric M-theory compactifications to $AdS_5$. These describe spontaneously broken higher-form gauge symmetries in the bulk. Different choices of boundary conditions for the BF terms yield dual field theories with distinct global discrete symmetries. We discuss in detail these symmetries and their 't Hooft anomalies for 4d $\mathcal N = 1$ SCFTs arising from M5-branes wrapped on a Riemann surface without punctures, including theories from M5-branes at a $\mathbb Z_2$ orbifold singularity. The anomaly polynomial is computed via inflow and contains background fields for discrete global 0-, 1-, and 2-form symmetries and continuous 0-form symmetries, as well as axionic background fields. The latter are properly interpreted in the context of anomalies in the space of coupling constants.

==> topmatter.tex <==
\def\check{\textbf{CHECK!}}


%\usepackage{array,setspace,mathrsfs,amsfonts,amsmath,yfonts,dsfont,bbm,colonequals,youngtab,mathabx}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}



%\usepackage{graphicx}
%\usepackage{epsfig}
%\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{hyperref}
%\usepackage[height=8.8in,width=6.45in]{geometry}
%\def\baselinestretch{1.05}

\numberwithin{equation}{section}
\newtheorem{conj}{Conjecture}
\newtheorem{thm}{Theorem}

\def\NO#1#2{{\rm NO}(#1,#2)}
\def\CB#1{$\clubsuit$ {\bf #1} $\clubsuit$}
\def\inc#1{\vcenter{\hbox{\includegraphics[scale=.25]{#1}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\ceq{\colonequals}
\def\eqc{\equalscolon}
\def\eqq{\equiv}
\def\leqs{\leqslant}
\def\geqs{\geqslant}
\def\vph{\varphi}
\def\vth{\vartheta}
\def\g{\gamma}
\def\G{\Gamma}
\def\th{\theta}
\def\Th{\Theta}
\def\tpdf{\texorpdfstring}

\DeclarePairedDelimiterX\MeijerM[3]{\lparen}{\rparen}%
{\begin{smallmatrix}#1 \\ #2\end{smallmatrix}\delimsize\vert\,#3}

\def\zeromode#1{o\left(#1\right)}

\newcommand\MeijerG[8][]{%
  G^{\,#2,#3}_{#4,#5}\MeijerM[#1]{#6}{#7}{#8}}

\WithSuffix\newcommand\MeijerG*[7]{%
  G^{\,#1,#2}_{#3,#4}\MeijerM*{#5}{#6}{#7}}


%\def\VnoH{\VV_{\cancel{\rm H}}}
\def\VH{\VV_0}
\def\VnoH{\VV_+}
\def\VSch{\mathcal{V}_{\rm Sch}}

\newcommand{\suup}{2}
\newcommand{\sudown}{1}
\def\diag{\mathop{\mathrm{diag}}\nolimits}
\def\tr{\mathop{\mathrm{tr}}\nolimits}
\def\rank{\mathop{\mathrm{rank}}\nolimits}
\def\CP{\mathbb{CP}}
\def\GL{\mathrm{GL}}
\def\SL{\mathrm{SL}}
\def\SU{\mathrm{SU}}
\def\SO{\mathrm{SO}}
\def\USp{\mathrm{USp}}
\def\UU{\mathrm{U}}
\def\PE{\mathrm{PE}}
\def\bC{\mathbb{C}}
\def\bR{\mathbb{R}}
\def\bZ{\mathbb{Z}}
\def\cH{\mathcal{H}}
\def\cDI{\mathcal{DI}}
\def\cN{\mathcal{N}}
\def\cV{\mathbb{V}}
\def\fk{\mathfrak{k}}
\def\fg{\mathfrak{g}}
\def\fh{\mathfrak{h}}
\def\sN{\text{\sffamily N}}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\vev#1{\langle#1\rangle}
\def\Hyp{\mathcal{V}}
\def\half{\frac12}
\def\S{{\mathbb S}}


\def\Vir{{\rm Vir}}
\def\AD{{\rm AD}}
\def \Rf{\mf{R}}

\def \beg#1{\begin{#1}} %This is a hack for my compiler -- doesn't have any adverse effects in general
\def \be{\beg{equation}}
\def \bea{\beg{eqnarray}}
\def \eea{\end{eqnarray}}
\def \ee{\end{equation}}

\def \a{\alpha}
\def \b{\beta}
\def \D{\Delta}

\def \PE{\mathrm{P.E.}}
%\def \NO#1{\mathop{:}\nolimits\!#1\!\mathop{:}\nolimits}
\def \goodchi{\protect\raisebox{1pt}{$\chi$}}
\def \qq{\mathbbmtt{Q}\,}
\def \Qt{\wt\QQ}
\def \St{\wt\SS}
\def \Lh{\widehat{L}}
\def \Lb{\overline{L}}
\def \af{\mf{a}}
\def \df{\mf{d}}
\def \ef{\mf{e}}
\def \gf{\mf{g}}
\def \uf{\mf{u}}
\def \glf{\mf{gl}}
\def \slf{\mf{sl}}
\def \suf{\mf{su}}
\def \sof{\mf{so}}
\def \spf{\mf{sp}}
\def \psuf{\mf{psu}}
\def \uspf{\mf{usp}}
\def \ospf{\mf{osp}}
\def \of{\mf{o}}
\def \ef{\mf{e}}
\def \hhf{\mf{h}}
\def \ceq{\colonequals}
\def \bs#1{$\clubsuit${\bf #1}$\clubsuit$}
\def \restr#1#2{{\left.\kern-\nulldelimiterspace#1\vphantom{\big|}\right|_{#2}}}

\def \Poincare{Poincar\'e}

\def \ll{\lambda}

\def \ba{{\bf a}}
\def \bb{{\bf b}}
\def \bc{{\bf c}}
\def \bd{{\bf d}}

\def \bA{{\bf A}}
\def \bB{{\bf B}}
\def \bC{{\bf C}}
\def \bD{{\bf D}}
\def \bOn{{\bf 1}}
\def \bTw{{\bf 2}}
\def \bTh{{\bf 3}}
\def \bFo{{\bf 4}}
\def \bFi{{\bf 5}}
\def \cd{{\tilde c}}

\def \hf{\frac12}
\def \qt{\frac14}

\def \mf{\mathfrak}
\def \lb{\lbrack}
\def \rb{\rbrack}
\def \nn{\nonumber}
\def \ph{\phantom}
\def \wt{\widetilde}
\def \wh{\widehat}
\def \ol{\overline}
\def \eg{{\it e.g.}}
\def \ie{{\it i.e.}}
\def \cf{{\it cf.}}
\def \Tr{{\rm Tr}}
\def \STr{{\rm STr}}
\def \til{\tilde}
\def \pr{\prime}
\def \zb{{\bar z}}
\def \db{\ol{\partial}}
\def \d{\partial}
\def \dag{\dagger}

\def \Ab{\mathbb{A}}
\def \Cb{\mathbb{C}}
\def \Eb{\mathbb{E}}
\def \Fb{\mathbb{F}}
\def \Hb{\mathbb{H}}
\def \Kb{\mathbb{K}}
\def \Mb{\mathbb{M}}
\def \Nb{\mathbb{N}}
\def \Ob{\mathbb{O}}
\def \Qb{\mathbb{Q}}
\def \Rb{\mathbb{R}}
\def \Sb{\mathbb{S}}
\def \Zb{\mathbb{Z}}


\def \AA{\mathcal{A}}
\def \BB{\mathcal{B}}
\def \CC{\mathcal{C}}
\def \DD{\mathcal{D}}
\def \EE{\mathcal{E}}
\def \FF{\mathcal{F}}
\def \GG{\mathcal{G}}
\def \HH{\mathcal{H}}
\def \II{\mathcal{I}}
\def \JJ{\mathcal{J}}
\def \KK{\mathcal{K}}
\def \LL{\mathcal{L}}
\def \MM{\mathcal{M}}
\def \NN{\mathcal{N}}
\def \OO{\mathcal{O}}
\def \PP{\mathcal{P}}
\def \QQ{\mathcal{Q}}
\def \RR{\mathcal{R}}
\def \SS{\mathcal{S}}
\def \TT{\mathcal{T}}
\def \UU{\mathcal{U}}
\def \VV{\mathcal{V}}
\def \WW{\mathcal{W}}
\def \XX{\mathcal{X}}
\def \YY{\mathcal{Y}}
\def \ZZ{\mathcal{Z}}


\def \RRR{\mathfrak{R}}

